Detecting Hidden Webcams with Delay-Tolerant Similarity of Simultaneous Observation

Small, low-cost, wireless cameras are becoming increasingly commonplace making surreptitious observation of people more difficult to detect. Previous work in detecting hidden cameras has only addressed limited environments in small spaces where the user has significant control of the environment. To address this problem in a less constrained scope of environments, we introduce the concept of similarity of simultaneous observation where the user utilizes a camera (Wi-Fi camera, camera on a mobile phone or laptop) to compare timing patterns of data transmitted by potentially hidden cameras and the timing patterns that are expected from the scene that the known camera is recording. To analyze the patterns, we applied several similarity measures and demonstrated an accuracy of over 87% and and F1 score of 0.88 using an efficient threshold-based classification. We used our data set to train a neural network and saw improved results with accuracy as high as 97% and an F1 score over 0.95 for both indoors and outdoors settings. We further extend this work against an attacker who is capable of delaying when the video is sent. With the new approach, we see increased F1 scores above 0.98 for the original data and delayed data. From these results, we conclude that similarity of simultaneous observation is a feasible method for detecting hidden wireless cameras that are streaming video of a user. Our work removes significant limitations that have been put on previous detection methods.

==> appendices.tex <==

\appendices

\section{Tables of Results}
\label{sec:appendixa}

%TODO:  Put the tables here
\input{tables/dual_camera.cc.tex}

\input{tables/dual_camera.kld.n.jsd.tex}

\input{tables/mobile_record_video.dtw.tex}

\input{tables/mobile_record_video.kld.n.jsd.tex}

==> tables/confusion_matrix.tex <==
\begin{table}[h]

\definecolor{fp}{RGB}{190, 186, 252}
\definecolor{tp}{RGB}{252, 153, 153}
\definecolor{tn}{RGB}{184, 237, 177}
\definecolor{fn}{RGB}{255, 209, 135}




\footnotesize
\centering
 \begin{tabular}{cp{3cm}<{\raggedright}|p{3cm}<{\raggedright}|p{3cm}<{\raggedright}|}\cline{3-4}
   && \multicolumn{2}{c|}{\bfseries True condition} \\\hline
   \multicolumn{1}{|c|}{\multirow{8}{*}{Predicted condition}} & Total population & Hidden Wi-Fi camera & Not hidden Wi-Fi camera \\\cline{2-4}
   \multicolumn{1}{|c|}{} & Predicted as hidden Wi-Fi camera &\cellcolor{tp} \multirow{3}{*}{\bfseries True positive} &\cellcolor{fp} \bfseries \multirow{3}{*}{False positive} \\\cline{2-4}
   \multicolumn{1}{|c|}{} & Predicted as not hidden Wi-Fi camera &\cellcolor{fn} \multirow{3}{*}{\bfseries False negative} &\cellcolor{tn} \bfseries \multirow{3}{*}{True negative}\\\hline
   		\noalign{\vskip 1mm}   
 \end{tabular}
 \caption{Confusion matrix.}
 \label{confusion}
\end{table}

==> tables/confusion_matrix_derivations.tex <==
\begin{table}[h]
\setlength{\cellspacetoplimit}{0.5cm}
\setlength{\cellspacebottomlimit}{0.5cm}
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\definecolor{AvgError}{rgb}{0.99,0.76,0.8}
\definecolor{AvgAccuracy}{rgb}{0.94,0.86,0.51}
\footnotesize
\centering
 \begin{tabular}{|Sc|Sc|}\hline  
   Accuracy  & $\displaystyle\frac{\mathit{TP} + \mathit{TN}}{\mathit{TP} + \mathit{FP} + \mathit{TN} + \mathit{FN}}$ \\\hline
   Error     & $1 - \mathrm{Accuracy}$ \\\hline
   Precision & $\displaystyle\frac{\mathit{TP}}{\mathit{TP} + \mathit{FP}}$ \\\hline
   Recall    & $\displaystyle\frac{\mathit{TP}}{\mathit{TP} + \mathit{FN}}$ \\\hline
   F1 score  & $\displaystyle2\times\frac{\mathrm{Precision}\times\mathrm{Recall}}{\mathrm{Precision}+\mathrm{Recall}}$ \\\hline
   		\noalign{\vskip 1mm}   
 \end{tabular}
 \caption{Derivations from confusion matrix.}
 \label{deri-con}
\end{table}

==> tables/data_collection.tex <==
\begin{table*}[h]
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\centering
\footnotesize
\begin{tabular}{|c|c|c|c|c|}\hline
   \multicolumn{5}{|c|}{\bfseries\cellcolor{header}Data collection} \\\hline\hline
   \multicolumn{2}{|c|}{\bfseries\cellcolor{section1}Wi-Fi camera} & \multicolumn{2}{c|}{\bfseries\cellcolor{section1}Recorded video} & \bfseries\cellcolor{section2}Other non-spying camera traffics \\\hline
   \multicolumn{2}{|c|}{No motion} & \multicolumn{2}{c|}{No motion} & Skype \\\hline
   \multirow{3}{*}{Motion} &   0 degree  & \multirow{3}{*}{720p} &   0 degree  & YouTube    \\\hline
                           &  90 degrees &                       &  90 degrees & YouTube TV \\\hline
                           & 180 degrees &                       & 180 degrees & Amazon TV  \\\hline
   
   \multicolumn{2}{|c|}{Campus} & \multirow{3}{*}{1080p} &   0 degree  & Switch gaming       \\\hline
   \multicolumn{2}{|c|}{      } &                        &  90 degrees & Normal browsing     \\\hline
   \multicolumn{2}{|c|}{      } &                        & 180 degrees & Video downloading   \\\hline
   Courtyard  & 0 degrees &    Courtyard            & 0 degrees &   \\\hline
     & 90 degrees             &      & 90 degrees &   \\\hline
   \multicolumn{5}{|c|}{\bfseries\cellcolor{header}Total} \\\hline
   \multicolumn{2}{|c|}{$305$}  & \multicolumn{2}{c|}{$376$} & $260$ \\\hline
   		\noalign{\vskip 1mm}   
\end{tabular}

 \caption{Data collections of the experiment.}
 \label{data-collection table}
\end{table*}

==> tables/dual_camera.cc.tex <==
\begin{table*}[h]
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\definecolor{highlight}{rgb}{0.94,0.86,0.51}
\definecolor{bad-highlight}{RGB}{242, 160, 157}

\footnotesize
\centering
%\begin{minipage}{0.4\paperwidth}
 \begin{tabular}{|c|c|c|c|}\hline
   \multicolumn{2}{|c|}{\bfseries\cellcolor{header}Testing samples} & \bfseries\cellcolor{header}Average & \bfseries\cellcolor{header}Standard deviation \\\hline\hline
   
  \multicolumn{4}{|l|}{\cellcolor{section1}\bfseries Wi-Fi camera} \\\hline
  \multicolumn{2}{|c|}{\cellcolor{highlight}No motion}       &\cellcolor{highlight}  $0.3037$ &\cellcolor{highlight}  $0.1718$ \\\hline
  \multirow{3}{*}{Motion} &   0 degree  &  $0.6028 $ & $0.1725$ \\\cline{2-4}
                          &  90 degrees &  $0.3865 $ & $0.3175$ \\\cline{2-4}
                          & 180 degrees &  $0.4027 $ & $0.2109$ \\\hline
  \multicolumn{2}{|c|}{Campus}          &  $0.3040 $ & $0.2726$ \\\hline
  
  \multicolumn{4}{|l|}{\cellcolor{section2}\bfseries Other non-spying camera traffics}\\\hline
  \multicolumn{2}{|c|}{Amazon TV}         & $-0.0101$           & $0.0975$ \\\hline
  \multicolumn{2}{|c|}{Switch gaming}     & $\phantom{-}0.0649$ & $0.0877$ \\\hline
  \multicolumn{2}{|c|}{Normal browsing}   & $-0.0256$           & $0.1523$ \\\hline
  \multicolumn{2}{|c|}{Skype}             & $\phantom{-}0.0020$ & $0.1436$ \\\hline
  \multicolumn{2}{|c|}{Video downloading} & $-0.0022$           & $0.0979$ \\\hline
  \multicolumn{2}{|c|}{YouTube}           & $-0.0070$           & $0.1106$ \\\hline
  \multicolumn{2}{|c|}{YouTube TV}        & $\phantom{-}0.0272$ & $0.0880$ \\\hline
  		\noalign{\vskip 1mm}   
 \end{tabular}
%  \end{minipage}
 % \begin{minipage}{0.6\paperwidth}
 
%   \begin{tabular}{|c|c|c|c|}\hline
%   \multicolumn{2}{|c|}{\bfseries\cellcolor{header}Testing samples} & \bfseries\cellcolor{header}Average & \bfseries\cellcolor{header}Standard deviation \\\hline\hline

%   \multicolumn{4}{|l|}{\cellcolor{section1}\bfseries Wi-Fi camera} \\\hline
%   \multicolumn{2}{|c|}{No motion}       & $0.011453722$ & $0.005228987$ \\\hline
%   \multirow{3}{*}{Motion} &   0 degree  & $0.005479047$ & $0.003783815$ \\\cline{2-4}
%                           &  90 degrees & $0.009357307$ & $0.014222304$ \\\cline{2-4}
%                           & 180 degrees & $0.007548263$ & $0.006156813$ \\\hline
%   \multicolumn{2}{|c|}{Campus}          & $0.028721493$ & $0.028825679$ \\\hline
  
%   \multicolumn{4}{|l|}{\cellcolor{section2}\bfseries Other non-spying camera traffics}\\\hline
%   \multicolumn{2}{|c|}{Amazon TV}         & $0.069038229$ & $0.026416606$ \\\hline
%   \multicolumn{2}{|c|}{Switch gaming}     & $0.037086219$ & $0.015433377$ \\\hline
%   \multicolumn{2}{|c|}{Normal browsing}   & $8.394858985$ & $4.355179579$ \\\hline
%   \multicolumn{2}{|c|}{Skype}             & $0.038609769$ & $0.099741421$ \\\hline
%   \multicolumn{2}{|c|}{Video downloading} & $0.063745689$ & $0.055284152$ \\\hline
%   \multicolumn{2}{|c|}{YouTube}           & $1.471183735$ & $1.268920535$ \\\hline
%   \multicolumn{2}{|c|}{YouTube TV}        & $0.047435962$ & $0.015764356$ \\\hline
%  \end{tabular}
%  \end{minipage}
 
 
 \caption{Result of the CC for Wi-Fi camera-based detection model.}
 \label{wifi-cc}
 
\end{table*}


==> tables/dual_camera.kld.n.jsd.tex <==
\begin{table*}[h]
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{header2}{rgb}{0.8,0.8,0.8}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\definecolor{highlight}{rgb}{0.94,0.86,0.51}
\definecolor{bad-highlight}{RGB}{242, 160, 157}

\centering
\footnotesize
\begin{tabular}{|c|c|c|>{\centering\arraybackslash}p{1.8cm}|c|>{\centering\arraybackslash}p{1.8cm}|}\hline
  \multicolumn{2}{|c|}{\cellcolor{header}} & \multicolumn{2}{c|}{\bfseries\cellcolor{header} KLD} & \multicolumn{2}{c|}{\bfseries\cellcolor{header} JSD} \\\hhline{|>{\arrayrulecolor{header}}--%
  >{\arrayrulecolor{black}}|----}
  \multicolumn{2}{|c|}{\cellcolor{header}\bfseries Testing samples}& \bfseries\cellcolor{header2}\multirow{2}{*}{Average} & \bfseries\cellcolor{header2}Standard deviation & \bfseries\cellcolor{header2}\multirow{2}{*}{Average} & \bfseries\cellcolor{header2}Standard deviation \\\hline\hline
  
  \multicolumn{6}{|l|}{\cellcolor{section1}\bfseries Wi-Fi camera} \\\hline
  \multicolumn{2}{|c|}{\cellcolor{highlight}No motion}       &\cellcolor{highlight} $0.0114$ &\cellcolor{highlight} $0.0052$ &\cellcolor{highlight} $0.0028$ &\cellcolor{highlight} $0.0012$ \\\hline
  \multirow{3}{*}{Motion} &   0 degree  & $0.0054$ & $0.0037$ & $0.0013$ & $0.0009$ \\\cline{2-6}
                          &  90 degrees & $0.0093$ & $0.0142$ & $0.0022$ & $0.0024$ \\\cline{2-6}
                          & 180 degrees & $0.0075$ & $0.0061$ & $0.0018$ & $0.0013$ \\\hline
  \multicolumn{2}{|c|}{Campus}          & $0.0287$ & $0.0288$ &\cellcolor{highlight} $0.0073$ &\cellcolor{highlight} $0.0073$ \\\hline
  
  \multicolumn{6}{|l|}{\cellcolor{section2}\bfseries Other non-spying camera traffics}\\\hline
  \multicolumn{2}{|c|}{Amazon TV}         & $0.0690$ & $0.0264$ & $0.0171$ & $0.0064$\\\hline
  \multicolumn{2}{|c|}{Switch gaming}     & $0.0370$ & $0.0154$ & $0.0086$ & $0.0034$\\\hline
  \multicolumn{2}{|c|}{Normal browsing}   & $8.3948$ & $4.3551$ & $0.3569$ & $0.1180$\\\hline
  \multicolumn{2}{|c|}{Skype}             & $0.0386$ & $0.0997$ & $0.0090$ & $0.0199$\\\hline
  \multicolumn{2}{|c|}{Video downloading} & $0.0637$ & $0.0552$ & $0.0151$ & $0.0121$\\\hline
  \multicolumn{2}{|c|}{YouTube}           & $1.4711$ & $1.2689$ & $0.2916$ & $0.1468$\\\hline
  \multicolumn{2}{|c|}{YouTube TV}        & $0.0474$ & $0.0157$ & $0.0118$ & $0.0038$\\\hline
  		\noalign{\vskip 1mm}   
 \end{tabular}
 
 \caption{Result of the KLD and JSD for Wi-Fi camera-based detection model.}
 \label{wifi-kld-n-jsd}
\end{table*}


==> tables/dual_camera.kld.tex <==
\begin{table}[h]
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\footnotesize
\centering
 \begin{tabular}{|c|c|c|c|}\hline
   \multicolumn{2}{|c|}{\bfseries\cellcolor{header}Testing samples} & \bfseries\cellcolor{header}Average & \bfseries\cellcolor{header}Standard deviation \\\hline\hline

  \multicolumn{4}{|l|}{\cellcolor{section1}\bfseries Wi-Fi camera} \\\hline
  \multicolumn{2}{|c|}{No motion}       & $0.0114$ & $0.0052$ \\\hline
  \multirow{3}{*}{Motion} &   0 degree  & $0.0054$ & $0.0037$ \\\cline{2-4}
                          &  90 degrees & $0.0093$ & $0.0142$ \\\cline{2-4}
                          & 180 degrees & $0.0075$ & $0.0061$ \\\hline
  \multicolumn{2}{|c|}{Campus}          & $0.0287$ & $0.0288$ \\\hline
  
  \multicolumn{4}{|l|}{\cellcolor{section2}\bfseries Other non-spying camera traffics}\\\hline
  \multicolumn{2}{|c|}{Amazon TV}         & $0.0690$ & $0.0264$ \\\hline
  \multicolumn{2}{|c|}{Switch gaming}     & $0.0370$ & $0.0154$ \\\hline
  \multicolumn{2}{|c|}{Normal browsing}   & $8.3948$ & $4.3551$ \\\hline
  \multicolumn{2}{|c|}{Skype}             & $0.0386$ & $0.0997$ \\\hline
  \multicolumn{2}{|c|}{Video downloading} & $0.0637$ & $0.0552$ \\\hline
  \multicolumn{2}{|c|}{YouTube}           & $1.4711$ & $1.2689$ \\\hline
  \multicolumn{2}{|c|}{YouTube TV}        & $0.0474$ & $0.0157$ \\\hline
  		\noalign{\vskip 1mm}   
 \end{tabular}
 \caption{Result of the KLD for Wi-Fi camera-based detection model.}
 \label{wifi-kld}
\end{table}


==> tables/grid_search.tex <==
\begin{table*}[h]
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{subheader}{rgb}{0.8,0.8,0.8}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\definecolor{AvgError}{rgb}{0.99,0.76,0.8}
\definecolor{AvgAccuracy}{rgb}{0.94,0.86,0.51}
\definecolor{highlight}{rgb}{0.94,0.86,0.51}

\footnotesize
\centering
 \begin{tabular}{|c|>{\centering}p{1.5cm}|>{\centering}p{2cm}|>{\centering}p{3cm}|c|c|}\hline
   \multicolumn{4}{|c|}{\bfseries\cellcolor{header}ANN models} & \cellcolor{AvgAccuracy} & \cellcolor{AvgError} \\\hhline{----%
   >{\arrayrulecolor{AvgAccuracy}}-%
   >{\arrayrulecolor{black}}|%
   >{\arrayrulecolor{AvgError}}-%
   >{\arrayrulecolor{black}}|%
   }
   \bfseries\cellcolor{subheader}\multirow{2}{*}{Solver} & \centering\bfseries\cellcolor{subheader}Hidden layers & \bfseries\cellcolor{subheader} Neurons per layer & \bfseries\cellcolor{subheader} Activation function &  \cellcolor{AvgAccuracy}\bfseries Avg. Accuracy &  \cellcolor{AvgError}\bfseries Avg. Error \\\hline\hline
   \multicolumn{6}{|c|}{\bfseries\cellcolor{section1}Wi-Fi camera-based detection model} \\\hline
   Lbfgs & $3$ & $6$  & Identity & $91.136$ & $8.86$ \\\hline
   Lbfgs & $3$ & $7$  & Relu     & $91.364$ & $8.64$ \\\hline
   Lbfgs & $3$ & $5$  & Logistic & $92.273$ & $7.73$ \\\hline
   \cellcolor{highlight}Lbfgs &\cellcolor{highlight}$3$ &\cellcolor{highlight}$13$ &\cellcolor{highlight} Logistic &\cellcolor{highlight}$92.727$ &\cellcolor{highlight}$7.27$ \\\hline

   \multicolumn{6}{|c|}{\bfseries\cellcolor{section2}Mobile phone-based detection model} \\\hline
   Lbfgs & $3$ & $6$  & Identity & $84.630$ & $15.37$ \\\hline
   Lbfgs & $3$ & $8$  & Identity & $85.000$ & $15.00$ \\\hline
   Lbfgs & $3$ & $5$  & Identity & $86.111$ & $13.89$ \\\hline
   Lbfgs & $3$ & $10$ & Tanh     & $86.296$ & $13.70$ \\\hline
   Lbfgs & $3$ & $11$ & Tanh     & $86.481$ & $13.52$ \\\hline
   \cellcolor{highlight}Lbfgs & \cellcolor{highlight}$3$&\cellcolor{highlight}$14$ &\cellcolor{highlight} Logistic &\cellcolor{highlight}$87.037$&\cellcolor{highlight}$12.96$ \\\hline
   		\noalign{\vskip 1mm}   
 \end{tabular}
 \caption{Grid search on 10-fold cross validation.}
 \label{grid}
\end{table*}

==> tables/mobile_record_video.dtw.tex <==
\begin{table*}[h]
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\definecolor{highlight}{rgb}{0.94,0.86,0.51}
\definecolor{bad-highlight}{RGB}{242, 160, 157}

\footnotesize
\centering
 \begin{tabular}{|c|c|c|c|}\hline
   \multicolumn{2}{|c|}{\bfseries\cellcolor{header}Testing samples} & \bfseries\cellcolor{header}Average & \bfseries\cellcolor{header}Standard deviation \\\hline\hline
   
  \multicolumn{4}{|l|}{\cellcolor{section1}\bfseries Recorded video}   \\\hline
  \multicolumn{2}{|c|}{No motion}      & $11.330$           & $3.757$ \\\hline
  \multirow{3}{*}{720p}  &   0 degree  & $\phantom{0}9.284$ & $2.894$ \\\cline{2-4}
                         &  90 degrees & $\phantom{0}8.951$ & $2.004$ \\\cline{2-4}
                         & 180 degrees & $\phantom{0}8.412$ & $1.806$ \\\hline
  \multirow{3}{*}{1080p} &   0 degree  & $\phantom{0}8.680$ & $2.176$ \\\cline{2-4}
                         &  90 degrees & $\phantom{0}9.611$ & $1.679$ \\\cline{2-4}
                         & 180 degrees & $10.841$           & $6.356$ \\\hline

  \multicolumn{4}{|l|}{\cellcolor{section2}\bfseries Other non-spying camera traffics}\\\hline
  \multicolumn{2}{|c|}{Amazon TV}         & $13.237$ & $4.404$ \\\hline
  \multicolumn{2}{|c|}{Switch gaming}     & $10.573$ & $3.504$ \\\hline
  \multicolumn{2}{|c|}{Normal browsing}   & $22.983$ & $5.867$ \\\hline
  \multicolumn{2}{|c|}{Skype}             & $12.018$ & $6.626$ \\\hline
  \multicolumn{2}{|c|}{Video downloading} & $11.082$ & $3.572$ \\\hline
  \multicolumn{2}{|c|}{YouTube}           & $23.181$ & $6.491$ \\\hline
  \multicolumn{2}{|c|}{YouTube TV}        & $13.564$ & $4.158$ \\\hline
  		\noalign{\vskip 1mm}   
 \end{tabular}
 \caption{Result of the DTW for mobile phone-based detection model.}
 \label{mobile-dtw}
\end{table*}


==> tables/mobile_record_video.jsd.tex <==
\begin{table}[htbp]
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\footnotesize
\centering
 \begin{tabular}{|c|c|c|c|}\hline
  \multicolumn{2}{|c|}{\bfseries\cellcolor{header}Testing samples} & \bfseries\cellcolor{header}Average & \bfseries\cellcolor{header}Standard deviation \\\hline\hline
  
  \multicolumn{4}{|l|}{\cellcolor{section1}\bfseries Recorded video}   \\\hline
  \multicolumn{2}{|c|}{No motion}      & $0.0033$ & $0.0046$ \\\hline
  \multirow{3}{*}{720p}  &   0 degree  & $0.0010$ & $0.0011$ \\\cline{2-4}
                         &  90 degrees & $0.0270$ & $0.0265$ \\\cline{2-4}
                         & 180 degrees & $0.0019$ & $0.0022$ \\\hline
  \multirow{3}{*}{1080p} &   0 degree  & $0.0017$ & $0.0016$ \\\cline{2-4}
                         &  90 degrees & $0.0012$ & $0.0008$ \\\cline{2-4}
                         & 180 degrees & $0.0017$ & $0.0018$ \\\hline

  \multicolumn{4}{|l|}{\cellcolor{section2}\bfseries Other non-spying camera traffics}\\\hline
  \multicolumn{2}{|c|}{Amazon TV}         & $0.0156$ & $0.0061$ \\\hline
  \multicolumn{2}{|c|}{Switch gaming}     & $0.0077$ & $0.0033$ \\\hline
  \multicolumn{2}{|c|}{Normal browsing}   & $0.3545$ & $0.1170$ \\\hline
  \multicolumn{2}{|c|}{Skype}             & $0.0074$ & $0.0202$ \\\hline
  \multicolumn{2}{|c|}{Video downloading} & $0.0136$ & $0.0121$ \\\hline
  \multicolumn{2}{|c|}{YouTube}           & $0.2908$ & $0.1471$ \\\hline
  \multicolumn{2}{|c|}{YouTube TV}        & $0.0107$ & $0.0037$ \\\hline
  		\noalign{\vskip 1mm}   
 \end{tabular}
 \caption{Result of the JSD for mobile phone-based detection model.}
 \label{mobile-jsd}
\end{table}


==> tables/mobile_record_video.kld.n.jsd.tex <==
\begin{table*}[h]
\definecolor{header}{rgb}{0.7,0.7,0.7}
\definecolor{section1}{rgb}{0.74, 0.83, 0.9}
\definecolor{section2}{RGB}{240, 204, 176}
\definecolor{header2}{rgb}{0.8,0.8,0.8}
\definecolor{highlight}{rgb}{0.94,0.86,0.51}
\definecolor{bad-highlight}{RGB}{242, 160, 157}

\centering
\footnotesize

 \begin{tabular}{|c|c|c|>{\centering\arraybackslash}p{1.8cm}|c|>{\centering\arraybackslash}p{1.8cm}|}\hline
  \multicolumn{2}{|c|}{\cellcolor{header}} & \multicolumn{2}{c|}{\bfseries\cellcolor{header} KLD} & \multicolumn{2}{c|}{\bfseries\cellcolor{header} JSD} \\\hhline{|>{\arrayrulecolor{header}}--%
  >{\arrayrulecolor{black}}|----}
  \multicolumn{2}{|c|}{\cellcolor{header}\bfseries Testing samples}& \bfseries\cellcolor{header2}\multirow{2}{*}{Average} & \bfseries\cellcolor{header2}Standard deviation & \bfseries\cellcolor{header2}\multirow{2}{*}{Average} & \bfseries\cellcolor{header2}Standard deviation \\\hline\hline 
  
  \multicolumn{6}{|l|}{\cellcolor{section1}\bfseries Recorded video}   \\\hline
  \multicolumn{2}{|c|}{\cellcolor{highlight}No motion}      &\cellcolor{highlight} $0.01582$ &\cellcolor{highlight} $0.0267$ &\cellcolor{highlight} $0.0033$ &\cellcolor{highlight} $0.0046$ \\\hline
  \multirow{3}{*}{720p}  &   0 degree  & $0.0043$ & $0.0044$ & $0.0010$ & $0.0011$ \\\cline{2-6}
                         &  90 degrees & $0.0030$ & $0.0013$ & $0.0007$ & $0.0003$ \\\cline{2-6}
                         & 180 degrees & $0.0081$ & $0.0111$ & $0.0019$ & $0.0022$ \\\hline
  \multirow{3}{*}{1080p} &   0 degree  & $0.0069$ & $0.0066$ & $0.0017$ & $0.0016$ \\\cline{2-6}
                         &\cellcolor{highlight} 90 degrees &\cellcolor{highlight} $0.0050$ &\cellcolor{highlight} $0.0034$ &\cellcolor{highlight} $0.0012$ &\cellcolor{highlight} $0.0008$ \\\cline{2-6}
                         & 180 degrees & $0.0078$ & $0.0141$ & $0.0017$ & $0.0018$ \\\hline
  
  \multicolumn{6}{|l|}{\cellcolor{section2}\bfseries Other non-spying camera traffics}\\\hline
  \multicolumn{2}{|c|}{Amazon TV}         & $0.0627$ & $0.0247$ & $0.0156$ & $0.0061$ \\\hline
  \multicolumn{2}{|c|}{Switch gaming}     & $0.0335$ & $0.0150$ & $0.0077$ & $0.0033$ \\\hline
  \multicolumn{2}{|c|}{Normal browsing}   & $8.2647$ & $4.2918$ & $0.3545$ & $0.1170$ \\\hline
  \multicolumn{2}{|c|}{Skype}             & $0.0324$ & $0.1007$ & $0.0074$ & $0.0202$ \\\hline
  \multicolumn{2}{|c|}{Video downloading} & $0.0580$ & $0.0552$ & $0.0136$ & $0.0121$ \\\hline
  \multicolumn{2}{|c|}{YouTube}           & $1.4634$ & $1.2637$ & $0.2908$ & $0.1471$ \\\hline
  \multicolumn{2}{|c|}{YouTube TV}        & $0.0429$ & $0.0154$ & $0.0107$ & $0.0037$ \\\hline
  		\noalign{\vskip 1mm}   
 \end{tabular}
 \caption{Result of the KLD and JSD for mobile phone-based detection model.}
 \label{mobile-kld-n-jsd}
\end{table*}

